Filter Like You Test: Data-Driven Data Filtering for CLIP Pretraining

We introduce Filter Like You Test (FLYT), an algorithm for curating large-scale vision-language datasets that learns the usefulness of each data point as a pretraining example. FLYT trains a scoring model that learns to weigh each example's features using gradient signals from downstream tasks training sets. Based on FLYT, we implement Mixing-FLYT (M-FLYT), which takes the per-example scores generated by different scoring methods as features, and learns to unify them into a single score. FLYT naturally produces a distribution over the training examples, which we leverage through Soft Cap Sampling (SCS), a strategy for obtaining a filtered pretraining dataset from per-example probabilities that samples examples while preventing over-representation through a repetition penalty. Using these methods, we achieve 40.1% ImageNet zero-shot accuracy on the DataComp medium scale filtering benchmark, a 2% absolute accuracy increase over all previous results and a 5.5% increase over results that - like us - use only public resources. Our approach also yields 37.7\% on the average of 38 DataComp evaluation tasks, outperforming previous public-resource approaches by 0.4\%.

==> figures/figure-1.tex <==
\begin{figure*}[h]
	\centering 
	\begin{overpic}[width=1\textwidth]{figures/figure_1_1.pdf}
		% Add math expressions using \put(x,y){$math$}
		% (x,y) are percentages of the image width/height (0-100)
		\put(24.6,39.9){\textcolor{regularArrow}{$\boldsymbol{\featureExtractor}$}}
		\put(38,40.1){\textcolor{regularArrow}{$\boldsymbol{\scoringParams}$}}
		\put(51,40.5){\textcolor{regularArrow}{$\boldsymbol{\score}$}}
		\put(67.5,40.5){\textcolor{regularArrow}{$\boldsymbol{\weight}$}}
		\put(31.5,26.7){\textcolor{regularArrow}{$\boldsymbol{\refParams}$}}
		\put(57,27.5){\textcolor{regularArrow}{$\boldsymbol{\refFeatures(\sample)}$}}
		\put(9,35.6){\textcolor{regularArrow}{$\boldsymbol{\sample}$}}
		\put(9,8.3){\textcolor{regularArrow}{$\boldsymbol{\refSample}$}}
		\put(31.3,6.3){\textcolor{regularArrow}{$\boldsymbol{\updatedRefParams}$}}
		\put(56.3,7.6){\textcolor{regularArrow}{$\boldsymbol{\refFunction_{\updatedRefParams}(\refSample)}$}}
		\put(85.5,33.3){\textcolor{regularArrow}{$\boldsymbol{\weightedLossNoParams}$}}
		\put(84,5.9){\textcolor{regularArrow}{$\boldsymbol{\downstreamLossNoParams}$}}
		\put(77.8,15.8){\textcolor{scoringGradientArrow}{$\scalebox{0.85}{$\grad_\scoringParams \downstreamLossNoParams$}$}}
		\put(56.5,42.5){\textcolor{functionArrow}{$\scalebox{0.8}{$\softmax$}$}}
		\put(77.8,25.7){\textcolor{functionArrow}{$\scalebox{0.85}{$\grad_{\refParams}\weightedLossNoParams$}$}}
		\put(18.7,16.5){\textcolor{functionArrow}{$\scalebox{0.8}{$\updateStep(\grad_{\refParams}\weightedLossNoParams)$}$}}
		\put(38.8,47.3){\textcolor{scoringGradientArrow}{$\scalebox{0.8}{$\updateStep(\grad_{\scoringParams}\downstreamLossNoParams)$}$}}
		
	\end{overpic}
	
	\caption{\label{fig:flow}
	In each \ourmethod{} training loop, the \scoringModel{} takes features extracted from a batch of upstream data and generates a score for each example. These scores are converted to weights via softmax. A \referenceModel{} processes the upstream batch, and the resulting embeddings, together with the weights, are used to compute a weighted CLIP loss. The \referenceModel{} is then updated using gradients from this loss. Next, this updated \referenceModel{} processes downstream data to compute a downstream loss, which produces a gradient signal that passes through the updated \referenceModel{} all the way to the \scoringModel{} parameters.
		%\yair{Very nice figure! All the math in the figure should move to LaTeX, preferably rendered here directly and positioned on top of the figure. I suggest making all the boxes/circles/etc. smaller and putting the text on top and outside of each box, with the math symbol inside, and anyway write the English description before the math symbol. Another suggestion is to add a legend explaining what the different-colored arrows mean. It might also be nice using a different line thickness for the different type of arrows.} \mikey{What do you think now? The math is rendered here, the text outside looked messy, so we positioned it on top of the math inside. I wasn't sure about the legend, the red arrow for the gradient is not conceptually different from the light blue, it's just "more important"}
	} 
\end{figure*}
